Adaptive Federated Learning via Dynamical System Model

Hyperparameter selection is critical for stable and efficient convergence of heterogeneous federated learning, where clients differ in computational capabilities, and data distributions are non-IID. Tuning hyperparameters is a manual and computationally expensive process as the hyperparameter space grows combinatorially with the number of clients. To address this, we introduce an end-to-end adaptive federated learning method in which both clients and central agents adaptively select their local learning rates and momentum parameters. Our approach models federated learning as a dynamical system, allowing us to draw on principles from numerical simulation and physical design. Through this perspective, selecting momentum parameters equates to critically damping the system for fast, stable convergence, while learning rates for clients and central servers are adaptively selected to satisfy accuracy properties from numerical simulation. The result is an adaptive, momentum-based federated learning algorithm in which the learning rates for clients and servers are dynamically adjusted and controlled by a single, global hyperparameter. By designing a fully integrated solution for both adaptive client updates and central agent aggregation, our method is capable of handling key challenges of heterogeneous federated learning, including objective inconsistency and client drift. Importantly, our approach achieves fast convergence while being insensitive to the choice of the global hyperparameter, making it well-suited for rapid prototyping and scalable deployment. Compared to state-of-the-art adaptive methods, our framework is shown to deliver superior convergence for heterogeneous federated learning while eliminating the need for hyperparameter tuning both client and server updates.

==> Adaptive_fe_algorithm.tex <==
\section{Adaptive Forward-Euler Time-Step Selection}

\begin{algorithm}
\caption{Forward-Euler Adaptive Time-Step Selection}
\label{time step algo}
\begin{algorithmic}[1]
\STATE{\textbf{Input: }$\nabla f_i(\cdot)$,  $\ILi(t)$, $x_i(t)$, $\alpha\in(0,1)$, $\beta>1$, $\gamma>0$}
%\hspace*{\algorithmicindent} \textbf{Output: } \Delta t 
\STATE{$\Delta t \gets (\Delta t)_t$}
\WHILE{$\max(|LTE|) < \eta-\epsilon$ and  $f(\x(t+\Delta t))< f(\x(t))+c\Delta t \nabla f(\xt)$}
\STATE{$\Delta t = \beta \Delta t$}
\ENDWHILE
\WHILE{$\max(|LTE|) \geq \eta+\epsilon$ or  $f(\x(t+\Delta t))\geq f(\x(t))+c\Delta t\nabla f(\xt)$}
\STATE{$\Delta t = \alpha \Delta t$}
\ENDWHILE
\RETURN $\Delta t$ 
\end{algorithmic}

==> previous_works.tex <==
\section{Previous Works}

Federated learning in heterogeneous settings (with varying client learning rates and non-IID data distributions) has been shown to suffer from issues such as objective inconsistency [\cite{fednova}] and client drift [\cite{shi2022optimization}\cite{zhao2018federated}]. Prior methods have addressed these issues through techniques including aggregation step-size adjustments [\cite{feddyn, pathak2020fedsplit,  karimireddy2020scaffold, li2020federated}\cite{li2019convergence, malinovsky2023server, charles2020outsized}] or incorporating momentum into client updates [\cite{das2022faster, xu2022coordinating, khanduri2021stem}], as well as a Newton-like method [\cite{li2019feddane}].


One of the key challenges in developing effective federated learning algorithms is hyperparameter tuning. Prior studies have shown that federated learning performance is highly sensitive to hyperparameter choices such as learning rates, local update steps, and regularization terms [\cite{kim2023adaptive}\cite{feddyn, li2019convergence}]. Poor hyperparameter tuning can impact convergence and final accuracy especially under heterogeneity. However, hyperparameter tuning across multiple clients and servers is both computationally and resource intensive. This has motivated previous work that focused on adaptive updates for either server or clients.

Server-side adaptive methods adjust the learning rates and aggregation of central agents to account for system heterogeneity. For example, SCAFFOLD [\cite{karimireddy2020scaffold}] adaptively selects control variates to address data heterogeneity.
FedYogi, FedAdaGrad, FedADAM [\cite{reddi2020adaptive}] extend adaptive gradient methods like Yogi, AdaGrad, and Adam to the server-side updates to better handle noisy client updates in federated learning. FedExp [\cite{jhunjhunwala2023fedexp}] stabilizes convergence due to client drift using exponential moving average updates of client models.
 FedDyn [\cite{feddyn}] uses a dynamic regularizer in the server updates to prioritize fairness and stability. However, server-side methods often depend on prior knowledge or assumptions about client learning rates, limiting their ability to support client-specific and non-uniform step sizes. Moreover, these aggregation strategies introduce additional hyperparameters, which themselves impact convergence and stability of the global model.



Client-side approaches focus on modifying client update dynamics to handle local objective misalignment. FedProx [\cite{li2019convergence}] introduces a proximal term to constrain client updates. Other works like MOON [\cite{li2021model}] introduce contrastive learning objectives at the client to handle heterogeneity of data distributions.[\cite{kim2023adaptive}] develops an auto-tuning method that adaptively selects client learning rates based on local gradient information. Although these methods improve client optimization, they often cannot address all of the challenges of heterogeneous federated learning. Without coordinated server adaptation, client-side improvements alone can be prone to issues such as client drift, inconsistent objectives, and degraded convergence under heterogeneity.



We develop an end-to-end strategy that adaptively selected hyperparameters across \emph{both} the server and each client. Our method builds on the dynamical systems model introduced by [\cite{fedecado}], but unlike the original approach, we develop adaptive learning rates and momentum parameters to eliminate the need for manual hyperparameter tuning. \textbf{Our main contribution} is an end-to-end adaptive hyperparameter tuning framework that optimizes both server and client dynamics and momentum parameters. The resulting method accelerates convergence in the presence of data and client heterogeneity while being robust to hyperparameter choices. This reduces the need for manual tuning, making federated learning more reliable in practical deployments.

\GJ{To save space, you could merge the related work section into the introduction.}
